Scalable Synthesis of Verified Controllers in Deep Reinforcement Learning

There has been significant recent interest in devising verification techniques for learning-enabled controllers (LECs) that manage safety-critical systems. Given the opacity and lack of interpretability of the neural policies that govern the behavior of such controllers, many existing approaches enforce safety properties through shield, a dynamic monitoring-and-repairing mechanism that ensures a LEC does not emit actions that would violate desired safety conditions. These methods, however, have been shown to have significant scalability limitations because verification costs grow as problem dimensionality and objective complexity increase. In this paper, we propose a new automated verification pipeline capable of synthesizing high-quality safe controllers even when the problem domain involves hundreds of dimensions, or when the desired objective involves stochastic perturbations, liveness considerations, and other complex non-functional properties. Our key insight involves separating safety verification from neural controller training, and using pre-computed verified safety shields to constrain the training process. Experimental results over a range of high-dimensional benchmarks demonstrate the effectiveness of our approach in a range of stochastic linear time-invariant and time-variant systems.

==> notations.tex <==
\usepackage{booktabs, multirow} 
\usepackage{soul}
\usepackage[table]{xcolor}
\usepackage{changepage,threeparttable}

\begin{table}[!htp]\centering
\caption{Generated by Spread-LaTeX}\label{tab:}
\scriptsize
\begin{tabular}{lrr}\toprule
Notations &Explaination \\\midrule
$pi_{nn}$ &Neural network controller \\
$\Pi_{l}^{k}$ &Linear controller family which selects linear controller every k steps \\
$K_i$ &One linear controller \\
$\selector$ &Linear controllers selector \\
$\phi_{opt}$ &The optimal linear controller selector generated by Algorithm 1 \\
$R$ &Reinforcement learning reward \\
$\mathcal{S}_0$ &Initial state set \\
$\mathcal{S}_u$ &Unsafe state set \\
$\bar{\mathcal{S}}_u$ &Safe state set \\
$\mathcal{D}_x$ &Distribution of random variable x \\
$\rs{t}$ &Reachable set without considering stochasticity at time t \\
$\srs{t}$ &Reachable set considering stochasticity at time t \\
$A_t$ &System matrix at time t \\
$B_t$ &Control matrix at time t \\
$s_t$ &Sytem state at time t \\
$\dot{s}_t$ &First order derivative of system state at time t \\
$w$ &Transition noise term \\
$M$ &Max execution step of a system \\
$\Omega$ &The tree-structure search space of linear controller combination \\
$p_t$ &The percentage of safe states in the reachable set at time t \\
$\hat{p}_t$ &Lower bound for the percentage of safe states in the reachable set at time t \\
$\mathtt{Region}(s, w)$ &Under noise w, compute all the possible region around state s \\
$\mathcal{T}_t$ &Transformation matrix computed with $A_t$, $B_t$ and $\selector(\lcf, 0)$. \\
$\mathcal{T}_w$ &Transformation matrix of noise term $w$ \\
$\mathcal{T}_s$ &Transformation matrix of state $s$ \\
$\lbx$ &Over-approximated lower bound of random variable x \\
$\ubx$ &Over-approximated Upper bound of random variable x \\
$\epsilon_l$ &Lower boundaries of a bounded distribution \\
$\epsilon_h$ &Upper boundary of a bounded distribution \\
$\delta$ &$\epsilon_h - \epsilon_l$ \\
$f_t$ &The probability density function for reachable set $\srs{t}$ \\
$\rpub$ &The upper bound of $f_t$ \\
$\mathtt{PrefixSame}(\selector, t)$ &All the selectors with same ancestor to the given selector $\selector$ \\
$\mathtt{AllRSet}_t$ &All the reachable sets at tiime t w.r.t one linear controller family \\
$\mathtt{PhiRSet}_t$ &The reachable set generated by a selector $\selector$ at step t \\
$*$ &Convolution operation \\
$P_B$ &Purturbation matrix on control matrix $B$. \\
$P_L$ &Purturbation matrix on lower bound of safety constraints \\
$P_U$ &Purturbation matrix on upper bound of safety constraints \\
$g_t$ &Transformation for state \\
$h_t$ &Transformation for stochasitic noise \\
$\mathcal{A}_l$ &Overapproximation lower boundary \\
$\mathcal{A}_l$ &Overapproximation upper boundary \\
\bottomrule
\end{tabular}
\end{table}
